YouTube Recommendations Reinforce Negative Emotions: Auditing Algorithmic Bias with Emotionally-Agentic Sock Puppets

Personalized recommendation algorithms, like those on YouTube, significantly shape online content consumption. These systems aim to maximize engagement by learning users' preferences and aligning content accordingly but may unintentionally reinforce impulsive and emotional biases. Using a sock-puppet audit methodology, this study examines YouTube's capacity to recognize and reinforce emotional preferences. Simulated user accounts with assigned emotional preferences navigate the platform, selecting videos that align with their assigned preferences and recording subsequent recommendations. Our findings reveal reveal that YouTube amplifies negative emotions, such as anger and grievance, by increasing their prevalence and prominence in recommendations. This reinforcement intensifies over time and persists across contexts. Surprisingly, contextual recommendations often exceed personalized ones in reinforcing emotional alignment. These findings suggest the algorithm amplifies user biases, contributing to emotional filter bubbles and raising concerns about user well-being and societal impacts. The study emphasizes the need for balancing personalization with content diversity and user agency.

==> outout <==
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./youtube.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18>
(/usr/local/texlive/2021/texmf-dist/tex/latex/acmart/acmart.cls
Document Class: acmart 2020/11/15 v1.75 Typesetting articles for the Associatio
n for Computing Machinery
(/usr/local/texlive/2021/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2021/texmf-dist/tex/generic/xkeyval/xkvutils.tex
(/usr/local/texlive/2021/texmf-dist/tex/generic/xkeyval/keyval.tex))))
(/usr/local/texlive/2021/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amscls/amsart.cls
Document Class: amsart 2020/05/29 v2.20.6
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/totpages/totpages.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/everyshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/environ/environ.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/trimspaces/trimspaces.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/textcase/textcase.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/hyperxmp/hyperxmp.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/stringenc/stringenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifmtarg/ifmtarg.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/oberdiek/ifdraft.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/ifluatex.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/ifvtex.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/ncctools/manyfoot.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/ncctools/nccfoots.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftex/glyphtounicode.tex)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cmap/cmap.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fontenc.sty<<t1.cmap>>)
(/usr/local/texlive/2021/texmf-dist/tex/latex/libertine/libertine.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/ifxetex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/textcomp.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/fontaxes/fontaxes.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/libertine/LinLibertine_I.tex))
(/usr/local/texlive/2021/texmf-dist/tex/latex/inconsolata/zi4.sty
`inconsolata-zi4' v1.12, 2019/05/17 Text macros for Inconsolata (msharpe))
(/usr/local/texlive/2021/texmf-dist/tex/latex/newtx/newtxmath.sty
`newtxmath' v1.640, 2020/12/20 Math macros based originally on txfonts (msharpe
) (/usr/local/texlive/2021/texmf-dist/tex/latex/oberdiek/centernot.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kastrup/binhex.tex))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption-ams-smf.sto)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/float/float.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/comment/comment.sty
Excluding comment 'comment') Excluding comment 'CCSXML'
(/usr/local/texlive/2021/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty)
Special comment 'acks'
(/usr/local/texlive/2021/texmf-dist/tex/latex/libertine/T1LinuxLibertineT-TLF.f
d)) (/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/longtable.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/tabularx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/array.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/blindtext/blindtext.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/makecell/makecell.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cleveref/cleveref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/rotating.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/fixme/fixme.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/marginnote/marginnote.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tcolorbox/tcolorbox.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.te
x
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/utilities/pgfutil-common-li
sts.tex))
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/utilities/pgfkeysfiltered.c
ode.tex))
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.d
ef
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-p
df.def)))
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.
code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.
code.tex))
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex
)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.
tex
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic
.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigo
nometric.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.rando
m.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.compa
rison.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.
code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round
.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.
code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integ
erarithmetics.code.tex)))
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex)
) (/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/math/pgfint.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.co
de.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconst
ruct.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage
.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.co
de.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicst
ate.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransform
ations.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.cod
e.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.c
ode.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathproce
ssing.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.co
de.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.cod
e.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.cod
e.tex
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.
code.tex))
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.co
de.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretranspare
ncy.code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.
code.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.
tex)))
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.cod
e.tex)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.
tex)
(/usr/local/texlive/2021/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-0-65.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-1-18.sty)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tcolorbox/tcblistingsutf8.code.te
x
Library (tcolorbox): 'tcblistingsutf8.code.tex' version '4.42'
(/usr/local/texlive/2021/texmf-dist/tex/latex/tcolorbox/tcblistings.code.tex
Library (tcolorbox): 'tcblistings.code.tex' version '4.42'
(/usr/local/texlive/2021/texmf-dist/tex/latex/listings/listings.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/listings/listings.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tcolorbox/tcblistingscore.code.te
x
Library (tcolorbox): 'tcblistingscore.code.tex' version '4.42'
(/usr/local/texlive/2021/texmf-dist/tex/latex/tcolorbox/tcbprocessing.code.tex
Library (tcolorbox): 'tcbprocessing.code.tex' version '4.42'
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/shellesc.sty))))
(/usr/local/texlive/2021/texmf-dist/tex/latex/listingsutf8/listingsutf8.sty))

Package array Warning: Column X is already defined on input line 32.

Excluding comment 'screenonly' Include comment 'printonly'
Include comment 'anonsuppress'
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./youtube.aux

LaTeX Warning: Label `fig:h2.1:box' multiply defined.


LaTeX Warning: Label `fig:h2.1:box@cref' multiply defined.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/newtx/omlnxlmi.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/newtx/untxexa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/newtx/lmsntxsy.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/newtx/lmxntxexx.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/libertine/OT1LinuxLibertineT-TLF.
fd)<<ot1.cmap>><<oml.cmap>>
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/newtx/untxmia.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/newtx/untxsym.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/newtx/untxsyc.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./youtube.out) (./youtube.out)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/local/texlive/2021/texmf-dist/tex/latex/upquote/upquote.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/ltcaption.sty)
(./sections/0.abstract.tex)
(/usr/local/texlive/2021/texmf-dist/tex/latex/libertine/T1LinuxBiolinumT-TLF.fd
) (/usr/local/texlive/2021/texmf-dist/tex/latex/inconsolata/t1zi4.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/microtype/mt-msb.cfg)
(./sections/1.introduction.tex

Package natbib Warning: Citation `noauthor_social_2024' on page 1 undefined on 
input line 2.


Package natbib Warning: Citation `munger2022right' on page 1 undefined on input
 line 2.


Package natbib Warning: Citation `tufekci_opinion_2018' on page 1 undefined on 
input line 2.


Package natbib Warning: Citation `covington_deep_2016' on page 1 undefined on i
nput line 2.


Package natbib Warning: Citation `kleinberg_challenge_2024' on page 1 undefined
 on input line 2.


Package natbib Warning: Citation `cunningham_ranking_2023' on page 1 undefined 
on input line 2.


Package natbib Warning: Citation `cunningham_what_2024' on page 1 undefined on 
input line 2.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 7.


Package natbib Warning: Citation `chen_subscriptions_2023' on page 1 undefined 
on input line 7.


Package natbib Warning: Citation `hosseinmardi_causally_2024' on page 1 undefin
ed on input line 7.


Package natbib Warning: Citation `berger_what_2012' on page 1 undefined on inpu
t line 7.


Package natbib Warning: Citation `savolainen_delighting_2020' on page 1 undefin
ed on input line 7.


Package natbib Warning: Citation `gupta_predicting_2019' on page 1 undefined on
 input line 7.


Package natbib Warning: Citation `de_leon_sadness_2021' on page 1 undefined on 
input line 7.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 9.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 11.


Underfull \vbox (badness 10000) has occurred while \output is active [1.1{/usr/
local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
Underfull \vbox (badness 2277) has occurred while \output is active)
(./sections/2.0.background.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 11.


Package natbib Warning: Citation `covington_deep_2016' on page 2 undefined on i
nput line 12.

[2.2]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 19.


Package natbib Warning: Citation `kitroeff_why_2014' on page 3 undefined on inp
ut line 22.


Package natbib Warning: Citation `ruggiero_uses_2000' on page 3 undefined on in
put line 26.


Package natbib Warning: Citation `valentino_is_2008' on page 3 undefined on inp
ut line 26.


Package natbib Warning: Citation `robertson_negativity_2023' on page 3 undefine
d on input line 26.


Package natbib Warning: Citation `robertson_negativity_2023' on page 3 undefine
d on input line 26.


Package natbib Warning: Citation `fan_anger_2014' on page 3 undefined on input 
line 26.


Package natbib Warning: Citation `brady_emotion_2017' on page 3 undefined on in
put line 26.


Package natbib Warning: Citation `berger_arousal_2011' on page 3 undefined on i
nput line 26.


Package natbib Warning: Citation `crockett_moral_2017' on page 3 undefined on i
nput line 26.


Package natbib Warning: Citation `brady_mad_2020' on page 3 undefined on input 
line 26.


Package natbib Warning: Citation `carpenter_political_2020' on page 3 undefined
 on input line 26.


Package natbib Warning: Citation `ecker_psychological_2022' on page 3 undefined
 on input line 26.


Package natbib Warning: Citation `rathje_out-group_2021' on page 3 undefined on
 input line 26.


Package natbib Warning: Citation `baumeister_bad_2001' on page 3 undefined on i
nput line 26.


Underfull \vbox (badness 1817) has occurred while \output is active

Package natbib Warning: Citation `berger_what_2012' on page 3 undefined on inpu
t line 29.


Package natbib Warning: Citation `fan_anger_2014' on page 3 undefined on input 
line 29.


Package natbib Warning: Citation `brady_emotion_2017' on page 3 undefined on in
put line 29.


Package natbib Warning: Citation `berger_arousal_2011' on page 3 undefined on i
nput line 29.


Package natbib Warning: Citation `crockett_moral_2017' on page 3 undefined on i
nput line 29.


Package natbib Warning: Citation `brady_mad_2020' on page 3 undefined on input 
line 29.


Package natbib Warning: Citation `carpenter_political_2020' on page 3 undefined
 on input line 29.


Package natbib Warning: Citation `ecker_psychological_2022' on page 3 undefined
 on input line 29.


Package natbib Warning: Citation `habib_making_2022' on page 3 undefined on inp
ut line 30.


Package natbib Warning: Citation `noauthor_st_nodate' on page 3 undefined on in
put line 30.


Package natbib Warning: Citation `mccauley_mechanisms_2008' on page 3 undefined
 on input line 30.


Package natbib Warning: Citation `corner_mental_2018' on page 3 undefined on in
put line 30.


Package natbib Warning: Citation `rathje_out-group_2021' on page 3 undefined on
 input line 31.


Package natbib Warning: Citation `yardi_dynamic_2010' on page 3 undefined on in
put line 31.


Package natbib Warning: Citation `baumeister_bad_2001' on page 3 undefined on i
nput line 32.


Package natbib Warning: Citation `brady_emotion_2017' on page 3 undefined on in
put line 32.


Package natbib Warning: Citation `robertson_negativity_2023' on page 3 undefine
d on input line 32.


Package natbib Warning: Citation `del_vicario_echo_2016' on page 3 undefined on
 input line 32.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 36.


Package natbib Warning: Citation `slater_reinforcing_2007' on page 3 undefined 
on input line 36.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 38.


Package natbib Warning: Citation `goldenberg_amplification_2023' on page 3 unde
fined on input line 39.


Package natbib Warning: Citation `martel_reliance_2020' on page 3 undefined on 
input line 39.


Package natbib Warning: Citation `brady_emotion_2017' on page 3 undefined on in
put line 39.


Package natbib Warning: Citation `knutson_news_2024' on page 3 undefined on inp
ut line 39.


Package natbib Warning: Citation `martel_reliance_2020' on page 3 undefined on 
input line 41.


Package natbib Warning: Citation `brady_emotion_2017' on page 3 undefined on in
put line 41.


Package natbib Warning: Citation `knutson_news_2024' on page 3 undefined on inp
ut line 41.

) (./sections/2.1.related.tex
Underfull \vbox (badness 2277) has occurred while \output is active [3.3]

Package natbib Warning: Citation `ribeiro_amplification_2023-1' on page 4 undef
ined on input line 4.


Package natbib Warning: Citation `haroon_youtube_2022' on page 4 undefined on i
nput line 4.


Package natbib Warning: Citation `alfano_technologically_2021' on page 4 undefi
ned on input line 4.


Package natbib Warning: Citation `brown_echo_2022' on page 4 undefined on input
 line 4.


Package natbib Warning: Citation `ribeiro_auditing_2020' on page 4 undefined on
 input line 4.


Package natbib Warning: Citation `haroon_youtube_2022' on page 4 undefined on i
nput line 4.


Package natbib Warning: Citation `alfano_technologically_2021' on page 4 undefi
ned on input line 4.


Package natbib Warning: Citation `chen_subscriptions_2023' on page 4 undefined 
on input line 6.


Package natbib Warning: Citation `hosseinmardi_causally_2024' on page 4 undefin
ed on input line 6.


Package natbib Warning: Citation `hosseinmardi_examining_2021' on page 4 undefi
ned on input line 6.


Package natbib Warning: Citation `munger2022right' on page 4 undefined on input
 line 6.


Package natbib Warning: Citation `chen_subscriptions_2023' on page 4 undefined 
on input line 6.


Package natbib Warning: Citation `hosseinmardi_examining_2021' on page 4 undefi
ned on input line 6.


Package natbib Warning: Citation `munger2022right' on page 4 undefined on input
 line 6.


Underfull \vbox (badness 10000) has occurred while \output is active

Package natbib Warning: Citation `crockett_moral_2017' on page 4 undefined on i
nput line 10.


Package natbib Warning: Citation `mcloughlin_misinformation_2024' on page 4 und
efined on input line 10.


Package natbib Warning: Citation `brady_emotion_2017' on page 4 undefined on in
put line 10.


Package natbib Warning: Citation `rathje_out-group_2021' on page 4 undefined on
 input line 12.


Package natbib Warning: Citation `vosoughi_spread_2018' on page 4 undefined on 
input line 12.


Package natbib Warning: Citation `prollochs_emotions_2021' on page 4 undefined 
on input line 12.


Package natbib Warning: Citation `corbu_does_2020' on page 4 undefined on input
 line 12.

) (./sections/3.data.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 2.


Underfull \vbox (badness 1796) has occurred while \output is active [4.4]

Package natbib Warning: Citation `chandio_how_2024' on page 5 undefined on inpu
t line 20.


Package natbib Warning: Citation `luan_luanrtyoutubejs_2025' on page 5 undefine
d on input line 20.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 22.

(./sections/tables/data1.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 7.


(/usr/local/texlive/2021/texmf-dist/tex/latex/libertine/TS1LinuxLibertineT-TLF.
fd)

Package natbib Warning: Citation `boyd_development_2022' on page 5 undefined on
 input line 15.


Package natbib Warning: Citation `boyd_development_2022' on page 5 undefined on
 input line 16.


Package natbib Warning: Citation `boyd_development_2022' on page 5 undefined on
 input line 17.


Package natbib Warning: Citation `hutto_vader_2014' on page 5 undefined on inpu
t line 18.


Package natbib Warning: Citation `hutto_vader_2014' on page 5 undefined on inpu
t line 19.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 23.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 23.

)

LaTeX Warning: Reference `tab:videos' on page 1 undefined on input line 31.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 33.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 36.


Package natbib Warning: Citation `zhou_counting_2011' on page 5 undefined on in
put line 37.


Package natbib Warning: Citation `mcgrady_dialing_2023' on page 5 undefined on 
input line 37.

[5.5]) (./sections/4.H1.tex
Underfull \vbox (badness 1033) has occurred while \output is active

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 33.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 42.


Underfull \vbox (badness 1742) has occurred while \output is active [6.6]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 50.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 57.

(./sections/tables/h1-results.tex

LaTeX Warning: `!h' float specifier changed to `!ht'.

)
Underfull \vbox (badness 1622) has occurred while \output is active

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 76.

[7.7]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 92.


Class acmart Warning: A possible image without description on input line 106.


LaTeX Warning: `h' float specifier changed to `ht'.

) (./sections/5.H2.tex [8.8]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 20.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 28.

(./sections/tables/h2-results.tex)
Overfull \hbox (12.0pt too wide) in paragraph at lines 44--45
 [][] 

Class acmart Warning: A possible image without description on input line 47.

[9.9 <./sections/figures/H1.1.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 53.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 67.

) (./sections/6.H3.tex
Underfull \vbox (badness 6859) has occurred while \output is active [10.10 <./s
ections/figures/H2.pdf>]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 35.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 84.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 101.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 110.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 120.

[11.11] (./sections/tables/h3.2-results.tex)
(./sections/tables/h3.1-results.tex
Overfull \hbox (11.99767pt too wide) in paragraph at lines 4--18
 [][] 
)

Class acmart Warning: A possible image without description on input line 138.


LaTeX Warning: `h' float specifier changed to `ht'.

[12.12 <./sections/figures/H3.2.pdf>]) (./sections/7.discussion.tex
Underfull \vbox (badness 7186) has occurred while \output is active

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 8.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 10.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 12.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 17.


Package natbib Warning: Citation `covington_deep_2016' on page 13 undefined on 
input line 17.

[13.13]

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 19.


Package natbib Warning: Citation `habib_uncovering_2024' on page 14 undefined o
n input line 20.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 22.


Package natbib Warning: Citation `brady_emotion_2017' on page 14 undefined on i
nput line 25.


Package natbib Warning: Citation `martel_reliance_2020' on page 14 undefined on
 input line 27.


Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 32.


Package natbib Warning: Citation `thorburn_what_2022' on page 14 undefined on i
nput line 33.


Underfull \vbox (badness 10000) has occurred while \output is active

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 35.


Package natbib Warning: Citation `thorburn_what_2022' on page 14 undefined on i
nput line 36.


Package natbib Warning: Citation `massanari_gamergate_2017' on page 14 undefine
d on input line 36.


Package natbib Warning: Citation `alfano_technologically_2021' on page 14 undef
ined on input line 36.


Package natbib Warning: Citation `yu_nudging_2024' on page 14 undefined on inpu
t line 36.


Package natbib Warning: Citation `lukoff_how_2021' on page 14 undefined on inpu
t line 36.


Package natbib Warning: Citation `baughan_i_2022' on page 14 undefined on input
 line 36.


Package natbib Warning: Citation `news_what_2024' on page 14 undefined on input
 line 36.

[14.14])
No file youtube.bbl.
(./sections/8.appendix.tex

Package natbib Warning: Citation `stone_how_2015' on page 15 undefined on input
 line 7.

(./sections/tables/videos.tex
Underfull \hbox (badness 2707) in paragraph at lines 19--19
[]|\T1/LinuxLibertineT-TLF/m/n/8 (+20) I Built 4 Se-cret Rooms

Underfull \hbox (badness 1178) in paragraph at lines 23--23
\T1/LinuxLibertineT-TLF/m/n/8 (+20) tors clash over Trump's

Underfull \hbox (badness 3138) in paragraph at lines 25--25
[]|\T1/LinuxLibertineT-TLF/m/n/8 (+20) Why US elec-tions only

Underfull \hbox (badness 1789) in paragraph at lines 26--26
[]|\T1/LinuxLibertineT-TLF/m/n/8 (+20) RFK Jr. could win 2024

Underfull \hbox (badness 1629) in paragraph at lines 26--26
\T1/LinuxLibertineT-TLF/m/n/8 (+20) pres-i-den-tial elec-tion: Bo

Underfull \hbox (badness 4595) in paragraph at lines 29--30
[]|\T1/LinuxLibertineT-TLF/m/n/8 (+20) Polkadot and The Tale

Underfull \hbox (badness 5817) in paragraph at lines 29--30
\T1/LinuxLibertineT-TLF/m/n/8 (+20) of Blockchain by Irina

Underfull \hbox (badness 10000) in paragraph at lines 30--31
[]|\T1/LinuxLibertineT-TLF/m/n/8 (+20) Kerala

Underfull \hbox (badness 10000) in paragraph at lines 30--31
\T1/LinuxLibertineT-TLF/m/n/8 (+20) Blockchain
))

Package natbib Warning: There were undefined citations.

(/usr/local/texlive/2021/texmf-dist/tex/generic/stringenc/se-pdfdoc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/stringenc/se-utf8.def)

Class acmart Warning: Some images may lack descriptions.


Class acmart Warning: ACM keywords are mandatory for papers over two pages.


Class acmart Warning: ACM reference format is mandatory for papers over one pag
e.


Class acmart Warning: CCS concepts are mandatory for papers over two pages.


FiXme Summary: Number of notes: 0,
(FiXme)        Number of warnings: 0,
(FiXme)        Number of errors: 0,
(FiXme)        Number of fatal errors: 0,
(FiXme)        Total: 0.

[15.15] [16.16] [17.17] (./youtube.aux)

LaTeX Warning: There were undefined references.


LaTeX Warning: There were multiply-defined labels.

 )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/libertine/lbtn_7f4ce4.enc}{/usr/local/texlive/2021/tex
mf-dist/fonts/enc/dvips/libertine/lbtn_oexx6f.enc}{/usr/local/texlive/2021/texm
f-dist/fonts/enc/dvips/libertine/lbtn_25tcsq.enc}{/usr/local/texlive/2021/texmf
-dist/fonts/enc/dvips/libertine/lbtn_7grukw.enc}{/usr/local/texlive/2021/texmf-
dist/fonts/enc/dvips/libertine/lbtn_nh77jq.enc}{/usr/local/texlive/2021/texmf-d
ist/fonts/enc/dvips/inconsolata/i4-t1-4.enc}{/usr/local/texlive/2021/texmf-dist
/fonts/enc/dvips/libertine/lbtn_76gpa5.enc}</usr/local/texlive/2021/texmf-dist/
fonts/type1/public/inconsolata/Inconsolata-zi4r.pfb></usr/local/texlive/2021/te
xmf-dist/fonts/type1/public/newtx/LibertineMathMI.pfb></usr/local/texlive/2021/
texmf-dist/fonts/type1/public/newtx/LibertineMathMI5.pfb></usr/local/texlive/20
21/texmf-dist/fonts/type1/public/newtx/LibertineMathMI7.pfb></usr/local/texlive
/2021/texmf-dist/fonts/type1/public/libertine/LinBiolinumT.pfb></usr/local/texl
ive/2021/texmf-dist/fonts/type1/public/libertine/LinBiolinumTB.pfb></usr/local/
texlive/2021/texmf-dist/fonts/type1/public/libertine/LinBiolinumTI.pfb></usr/lo
cal/texlive/2021/texmf-dist/fonts/type1/public/libertine/LinLibertineT.pfb></us
r/local/texlive/2021/texmf-dist/fonts/type1/public/libertine/LinLibertineTB.pfb
></usr/local/texlive/2021/texmf-dist/fonts/type1/public/libertine/LinLibertineT
I.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/newtx/NewTXMI.pfb>
</usr/local/texlive/2021/texmf-dist/fonts/type1/public/newtx/NewTXMI7.pfb></usr
/local/texlive/2021/texmf-dist/fonts/type1/public/newtx/txexs.pfb></usr/local/t
exlive/2021/texmf-dist/fonts/type1/public/newtx/txmiaX.pfb></usr/local/texlive/
2021/texmf-dist/fonts/type1/public/txfonts/txsyb.pfb></usr/local/texlive/2021/t
exmf-dist/fonts/type1/public/newtx/txsys.pfb>
Output written on youtube.pdf (17 pages, 735223 bytes).
Transcript written on youtube.log.


==> sections/abstract.tex <==
Personalized recommendation algorithms, like those on YouTube, significantly shape online content consumption. These systems aim to maximize engagement by learning users' preferences and aligning content accordingly but may unintentionally reinforce impulsive and emotional biases. Using a sock-puppet audit methodology, this study examines YouTube's capacity to recognize and reinforce emotional preferences. Simulated user accounts with assigned emotional preferences navigate the platform, selecting videos that align with their assigned preferences and recording subsequent recommendations. Our findings reveal reveal that YouTube amplifies negative emotions, such as anger and grievance, by increasing their prevalence and prominence in recommendations. This reinforcement intensifies over time and persists across contexts. Surprisingly, contextual recommendations often exceed personalized ones in reinforcing emotional alignment. These findings suggest the algorithm amplifies user biases, contributing to emotional filter bubbles and raising concerns about user well-being and societal impacts. The study emphasizes the need for balancing personalization with content diversity and user agency. 

==> sections/old_sections/3.rq1.tex <==
\para{Our Contributions}
While existing studies often demonstrate the presence of problematic patterns, the explanations behind such patterns are left unexplored. In our work, we take a more foundational approach by uncovering how recommendations are constructed and then pursue experiments that showcase how YouTube can reinforce user preferences, including their consumption behavior. First, we illustrate through a framework how recommendations are shaped by three key agents, user preferences, algorithm configurations, and collective user behavior. We then leverage this framework to uncover how YouTube responds to emotional and ideological preferences. Takeaways from these two investigations inform our discussion on the limitations of the preference-utility recommendation framework, responsibility YouTube has to its users, and the influence of collective user behavior on an individual's exposure to content.

% \para{RQ1: How personalized are YouTube recommendations?}
% Recommendations curated by an algorithm are shaped by many internal and external factors. This includes the user themselves, the configuration of the algorithm, and the collective behavior of the user-base. We investigate how user preferences shape YouTube personalization, more precisely, what proportion of recommendations are driven by personalization. Using a large scale sock-puppet experiment, we assign preferences to sock-puppets which communicate their preferences to YouTube via manipulating their watch history. Subsequently, the sock puppets records one million instances of recommendation as a response. Finally, we represent the recommendations in a latent space. This allows comparison between recommendations shown to different sock puppets for the same videos. We compare recommendations served to sock puppets with assigned preference with recommendations served to sock puppets with no preference to establish level of personalization. This allows explorations into what agencies are involved in serving recommendations—user agency, collective user agency, and algorithmic agency—and how these factors shape the perception of user preferences and content utilities by the platform.

\section{What Factors Shape YouTube Recommendations?} \label{sec:rq1}
Recommendations algorithms are complex systems that are influenced by multiple agents and mechanisms. Uncovering how recommendations are constructed is key to understanding their problematic outcomes. In this section, we perform experiments to uncover the anatomy of up-next recommendation on YouTube. More specifically, uncover the proportion of personalized recommendations driven by user preferences. We construct sock puppets that reveal different user preferences to the recommendation system and record the subsequent recommendation as the system's response. Comparing the recommendations served to the sock puppet with contextual recommendations, we measure the prevalence of personalized recommendations. In this section, we first outline the methodology used to create sock puppets that reveal their preferences and record recommendations. Then we describe the process of comparing sets of recommendations directly and within a latent space. Finally, we demonstrate our results and highlight the findings that inform our subsequent questions.

\subsection{Methods} \label{sec:rq2:methods}
The goal of our experiment is to uncover the prevalence of personalization within recommendations. To this end, we first obtain a large scale set of recommendations served to different user personas and then compare the recommendations with their contextual recommendations to determine the prevalence of personalization. In this section, we outline the methods used to obtain these recommendations and methods used to compare recommendations with contextual recommendations.

\para{Constructing sock puppets for YouTube.}
Researchers have extensively employed sock puppet methodologies to audit recommendations systems on YouTube and other content curation platforms. These methodologies rely on instrumenting web browsers, most commonly through tools such as selenium, to interact with the platform: communicating inputs and observing the responses. However, due to bot evasions techniques employed by platforms, performing large scale audit studies is expensive and time-consuming. YouTube being a cross-platform application (including TV, gaming consoles, handheld devices, and even fridges) has required a robust platform-agnostic backend to deliver comparable experiences across devices. To this end, YouTube had developed an internal hidden API, informally known as InnerTube API, that allows unrestricted and unthrottled access to basic internal functionality. Following the re-discovery of this API, researchers have used it to perform large scale exploratory studies that uncover the content libraries within the platform. In our work, we use the InnerTube API to perform sock puppet studies, auditing the recommendation algorithms within the platform. Specifically, from the API we use 4 endpoints to perform our audit studies: add to watch history, get recommendations, get homepage and sign-in. We discuss the InnerTube API and its consistency with actual YouTube recommendations in the appendix. Once we have built a system to watch videos and collect recommendations, we create \note{XXX} Google accounts using a Google Workspace account to perform our audits.

\para{Revealing sock puppet preferences to YouTube.}
Once the sock puppets are created, we assign them one of five preferences. These include four topical preferences: \textit{video games}, \textit{fitness}, \textit{news}, and two diametric political preferences: \textit{liberal}, \textit{conservative}. The topical preferences were selected because of their popularity and presence within the mainstream. \note{why is political used?}. Each preference is assigned a list of videos that are representative of the preference. For topical preferences, we obtain the lists of video by searching on YouTube for keywords related to the topic and fetching the results to curate a list of 100 videos each. Videos representing political preferences, liberal or conservative, are constructed using prior work investigating watching habits of users with either ideologies. Together, this results in 100 videos associated with each of the five preferences. Finally, sock puppets reveal their preferences by watching the videos associated with their preferences. 

\para{Collecting up-next recommendations for the sock puppets.}

\para{Representing the recommendations as latent embeddings}

\para{Measuring the differences between recommendations}

\subsection{Results}

- We have two key results:
the cdf for personalized and contextual recommendations. And then where are these recommendations coming from?

==> sections/old_sections/4.rq2.tex <==
\section{Does YouTube reinforce user preferences?}
Approximately three in four videos watched on YouTube are driven by the recommendation system. This makes the recommendations system responsible for a large portion of video options exposed to the user—consequently having the ability to shape user's beliefs and behaviors. Prior work have studied the YouTube recommendation system as a black box to uncover how they shape the recommendations and user behaviors \cite{haroon_youtube_2022, ribeiro_auditing_2020, hosseinmardi_causally_2024, hosseinmardi_examining_2021}. In our work, we seek to understand how YouTube recommendations, specifically personalized recommendations, are constructed as a result of the user's preferences. To this end, we perform experiments to uncover whether YouTube reinforces user preferences—specifically emotional preferences that might drive user's consumption behaviors. We use a sock puppet methodology to investigate whether YouTube reinforces user preferences characterized by emotional biases. Specifically, we uncover what are the mechanisms that facilitate this reinforcement, comparing reinforcement in contextual recommendations and personalized recommendations.

\subsection{Results}
\para{Overview of results.} 
In total, we conducted a comprehensive set of experiments to evaluate whether YouTube's recommendation system reinforces user preferences. We utilized seven preferences that were revealed to the recommendation system. For each preference, sock puppets were created in both signed-in and incognito configurations. The experiments were initiated from different seed videos drawn from either topical or random set of videos. We collect both contextual and personalized recommendations to evaluate whether YouTube recognizes user preferences, measure their reinforcement, and the uncover mechanisms through which this reinforcement is shaped. Findings from our experiments reveal two key results:
\begin{enumerate}
    \item Meaningful preferences are recognized, reinforced and ranked higher.
    \item Contextual recommendations are more reinforcing than personalized recommendations.
    \item Contextual recommendations reinforce preferences in the short-term.
\end{enumerate}
In the following sections, we demonstrate evidence that lead to these conclusions.

\subsubsection{Meaningful preferences are reinforced and ranked higher} 

\para{Sock puppets revealing user preferences capture preferences with higher utility than control sock puppets.}

\para{Negative, outrage, and anger are reinforced within news contexts.}

\para{Meaningless preferences are not reinforced.}

\para{Preferences are learned regardless of association with topic.}

\para{Content's utility is ranked higher in up-next recommendations}

\para{Congruent revelation of preference yields higher reinforcement.}

\para{Reinforcement increases with recommendation depth.}

\subsubsection{Contextual recommendations are more reinforcing than personalized recommendations} 
\para{Contextual recommendations are consistently more reinforcing.}
\para{Content's utility is (NOT) ranked higher in contextual recommendations.}
\para{Personalized recommendations limit reinforcements.}
\para{Contextual recommendations are driven by topic??}

Our experiments, sock puppets record the up-next recommendations served to them as they select and watch videos that align with their preferences. Comparing the videos exposed to treatment sock puppets with their control counterparts, we find treatment sock puppets are indeed exposed to videos that have higher utility to them. This validates our preference-utility framework, suggesting YouTube identifies preferences of a user through their selections and subsequently serves content that maximizes user's utility. More notably, we find this to be true only for \textit{meaningful} pairs of preferences and topics. Sock puppets with arbitrary preferences not found in the general population—namely, selecting videos with the highest percentage frequency of the letter \textit{h}—did not receive reinforcing recommendations any higher than their control counterparts. Additionally, we find some combination of preference and topic that were not enforced by the recommendations. We provide on explanation of this lack of reinforcement by limited representation in the collective user base. 
Analyzing the correlation between the rank of a video in the up-next recommendation and its utility score, we find a significant positive correlation for meaningful preferences. This further validates that YouTube's ranking and retreival mechanisms are designed to serve content that is aligned with the collective user behavior. We present our results for each of the preference and topic pair in the following table.

% \input{sections/tables/rq2-results}
\begin{table}[h]
\centering
\caption{Reinforcement of Impulsive Preferences Across Topics}
\label{tab:preference-reinforcement}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccc}
\hline
\textbf{Preference} & \textbf{Topic} & \textbf{Avg. Utility} & \textbf{Max Utility} & \textbf{Utility-Rank Correlation} & \textbf{Significant?} & \textbf{Notes} \\
\hline
Outrage & News & 0.78 & 0.93 & 0.71 & Yes & Strong reinforcement \\
Outrage & Gaming & 0.65 & 0.85 & 0.58 & Yes & Moderate reinforcement \\
Outrage & Fitness & 0.52 & 0.76 & 0.41 & Yes & Moderate reinforcement \\
\hline
Negative & News & 0.72 & 0.89 & 0.65 & Yes & Strong reinforcement \\
Negative & Gaming & 0.68 & 0.85 & 0.58 & Yes & Moderate reinforcement \\
Negative & Fitness & 0.45 & 0.71 & 0.32 & Yes & Weak reinforcement \\
\hline
Sad & News & 0.69 & 0.87 & 0.61 & Yes & Moderate reinforcement \\
Sad & Gaming & 0.58 & 0.79 & 0.47 & Yes & Moderate reinforcement \\
Sad & Fitness & 0.41 & 0.68 & 0.29 & Yes & Weak reinforcement \\
\hline
Anger & News & 0.76 & 0.91 & 0.68 & Yes & Strong reinforcement \\
Anger & Gaming & 0.70 & 0.88 & 0.62 & Yes & Strong reinforcement \\
Anger & Fitness & 0.55 & 0.78 & 0.44 & Yes & Moderate reinforcement \\
\hline
Group Identification & News & 0.81 & 0.95 & 0.74 & Yes & Very strong reinforcement \\
Group Identification & Gaming & 0.73 & 0.90 & 0.65 & Yes & Strong reinforcement \\
Group Identification & Fitness & 0.67 & 0.86 & 0.57 & Yes & Moderate reinforcement \\
\hline
Positive & News & 0.38 & 0.62 & 0.15 & No & No significant reinforcement \\
Positive & Gaming & 0.65 & 0.88 & 0.55 & Yes & Moderate reinforcement \\
Positive & Fitness & 0.78 & 0.93 & 0.70 & Yes & Strong reinforcement \\
\hline
H-frequency & News & 0.12 & 0.25 & 0.05 & No & No reinforcement \\
H-frequency & Gaming & 0.10 & 0.22 & 0.03 & No & No reinforcement \\
H-frequency & Fitness & 0.11 & 0.24 & 0.04 & No & No reinforcement \\
\hline
\end{tabular}%
}
\end{table}

Furthermore, our collection of up-next recommendations over the 100 watched allows us to observe the evolution of impulsive preferences over time. While due to the shortness of user session and the stochastic nature of the system, we refrain from making claims for rabit-holing effects, we find that the average utility of recommended videos increases over time, indicating a learning behavior of the system. These findings collectively demonstrate that YouTube's recommendation system does indeed reinforce meaningful impulsive preferences, potentially amplifying users' emotional biases over time. However, the system appears to be calibrated to recognize and respond to preferences that are common in the user population, rather than arbitrary or highly infrequent preferences.

\paraem{Reinforcement are driven by user preferences.} Up-next recommendations, as we discuss in \Cref{sec:background:algorithm}, are constructed through understanding the context of the video being watched along with user preferences. Therefore, findings from our previous analysis on up-next videos do isolate whether the reinforcing recommendations are driven by user preferences or the context of the video. Since it is possible the videos being selected and watched have naturally reinforcing contextual recommendations, driven by creator agency or collective user behavior. To rectify this, we analyze longitudinal changes in home page recommendations and the seed set of videos from which the sock puppets started. Due to the nature of home-page recommendations, the videos recommended on this surface are not influenced by any contextual recommendations—rather purely by the combination of learned user preferences and the YouTube's content library. Similarly, by observing recommendations on a consistent set of videos longitudinally, keeps the influence of contextual recommendations controlled, with changes in the recommendations purely reflecting changes in the learned preferences of the user. Using the same surfaces and methods as in measuring exposure from up-next videos, we find meaningful preferences are reinforced with the users being exposed to significantly higher reinforcing utility compared to control—on both the home page and the consistent set of seed videos. Taken together, we conclude the revealed and learned user preferences play a significant role in driving impulsive reinforcement. 

\paraem{Contextual recommendations drive higher reinforcement.} So far, we have discussed results derived from sock puppets that observed recommendations driven by user preferences, or user preferences combined with contextual recommendations. To this end, we discuss the influence of contextual recommendation on the reinforcement. For our sock puppets from prior analysis, in addition to collecting the recommendations they were exposed to, we also collect the contextual recommendation of the video. These recommendations are not influenced by the user-preference (there is some interference of user preference in this method that we have discussed in the sections before, namely the selection of the video being watched encodes some level of user preference. Surprisingly, comparing the exposed utilities of contextual recommendations with personalized recommendations, we found contextual recommendations to be consistently significantly more reinforcing. We found this to be true for all preference and topic pairs. Additionally, looking at the up-next exposure of the non-personalized sock puppet, we find a similar case of significantly higher reinforcement. We find these results to be of particular interest, suggesting the inclusion of penalization dampens the reinforcement of contextual recommendations.

\para{Discussion}

==> sections/old_sections/6.discussion.tex <==
\section{Discussion}

\para{Recommendation algorithms learn System 2 impulses from audience.}

\para{User preferences, collective user behavior, and creator dynamics play a big role in problematic outcomes}

\para{Algorithms can be tuned to serve user well-being.}
\thesis{This is beneficial for platforms as well, long-session users have declining retention.}


\para{Responsiblity vs Blame}
\thesis{talk about the clickbait example.}



\para{Giving what the users want}


\textbf{Jon Kleinberg | The challenge of understanding what users want}

Milkman, K.L., Rogers, T. and Bazerman, M.H. (2010) I’ll Have the Ice Cream Soon and the Vegetables Later: A Study of Online Grocery Purchases and Order Lead Time. Marketing Letters
- we find that as the delay between order completion and delivery increases, grocery customers spend less, order a higher percentage of “should” items (e.g., vegetables), and order a lower percentage of “want” items (e.g., ice cream), controlling for customer fixed effect

Highbrow Films Gather Dust: Time-Inconsistent Preferences and Online DVD Rentals
We predict and find that should DVDs (e.g., documentaries) are held significantly longer than want DVDs (e.g., action films) within-customer.
Our results suggest that present bias has a meaningful impact on choice in the field and that people may learn about their present bias with experience, and, as a result, gain the capacity to curb its influence.



TITLE: The Effect of Temporal Distance and Social Distance on the Choice of Consumers’ Preferences
Personal Choices over Time When choosing for themselves:

Now vs. Future Consumers are more likely to choose virtue products when making decisions for the future compared to now.


A better understanding of what users want

Understand the revealed preferences


\textbf{In extreme cases, when engagement is peak, users realize that they are addicted.}
% https://youtu.be/9A8r__NP_To?t=2828


Routes to improve this: autoplay vs preview. Jon Kleinberg

amazing citations for this in JOn Kleinberh pubs.

The Challenge of Understanding What Users Want: Inconsistent Preferences and Engagement Optimization

==> sections/old_sections/background.tex <==
\section{Background} \label{sec:background}
In this section, we outline concepts relevant to establishing the background, and significance of our work. We begin by explaining our current understanding of YouTube recommendation algorithms, as built by prior works and public documentation. Next, we outline the role of user preferences in recommendations, specifically, the different factors that drive user engagement behavior. 

\note{Somewhere here write about how we are only focusing on the up-next recommendations}
\subsection{Recommendation systems} \label{sec:background:algorithm}
YouTube has over 800 million videos \cite{citation} in its content library. A fundamental service YouTube provide to its users is the curation and recommendation of these videos. The mechanisms through which different platforms make recommendations is largely dependant on the platform's agenda, which typically prioritize maximizing user retention. This becomes an optimization problem for predicting the video a user will engage with \cite{watch time thing}. Based on our current understanding of recommendation systems and the theories these systems are based on, recommended videos are sources from three overlapping conceptual sets: videos that align with users preferences, videos within user network, and videos that are contextually relevant to the user. Different mechanisms construct these three sets that are combined to create a candidate set of videos. From this candidate set, videos are selected and ranked to present to the user. Taken together, at least 4 systems work together and separately to construct video recommendations. Exploring how these systems operate and shape the recommendations is crucial in understanding how problematic downstream outcomes emerge and can be mitigated. In the following sections, we illustrate our current current understand of these four systems. 

\para{Personalized recommendations}
Based on theories from behavioral economics, individuals are likely to engage with elements that aligns with their preferences \cite{recsys papers}. This requires recommendations systems to identify user preferences.  Early recommendation systems relied heavily on explicit user disclosures of preferences. This model, however, was limited in its agility, breadth, and ability to uncover all user preferences since individuals often struggle to articulate their own preferences accurately. Yet, when presented with choices, users can relatively easily identify items provides that align with their preferences. Therefore, by analyzing user interactions—specifically their choices and engagement with content—recommendation algorithms can infer user preferences. Note that these preferences are often represented as high dimensional latent vector constructed from the prior interactions of the users. Users with similar prior interactions will have similar vectors and there fore similar preferences. By tracking user selections from recommended content, algorithms can further refine their inference of user preferences, consequently optimizing recommendations for user engagement. Following inferring user preferences, recommendations systems select content that aligns with the user's preferences. In other words, recommendation systems select content that provides the most utility to the user. Similar to how user preferences can be represented as a single vector in a matrix of user interactions with content, content utility can be represented as the transpose of this matrix. This reflects the idea that content utility is defined by the users who engage with it: the more users with similar preferences engage with a piece of content, the higher its utility for other users with similar profiles. In the context of our study, this process of selected personalized recommendations is shaped by the 1) agency of the user—as they have direct control over their revealed preferences, and 2) the collective user behavior, as they shape how the content utility and user preferences are inferred.

\para{Contextual recommendations}
Contextual recommendations are characterized by their relevancy within a given context, and their likelihood to be engaged with next. Recommendation systems with limited access to user preferences, such as non-personalized advertising, watch-next recommendations on platforms with no history, or () rely on contextual recommendations. Building such recommendations follow a similar approach of using collaborative filtering and leveraging prior interactions of other users. When users with similar preferences consistently choose the same content, they signal its utility to the algorithm. Much like unsupervised learning, these inferences are not explicitly labeled; rather, the algorithm identifies patterns in the latent space, recognizing content with similar utility and users with similar preferences. Since contextual recommendations leverage collective user behavior,  the user base therefore effectively shapes the information a user is exposed to.

% \para{tag recommendations}
% \textit{look up why and how network recommendations are made.} 

\para{Up-next recommendations}
Up-next recommendations served to the user can be affiliated with one or more of the sets mentioned above. Following the candidate generation from all of these sets, the recommendation system selects twenty videos to rank them for the user in the up-next recommendation. The proportion of videos representing each set varies on the context of recommendations and is dependant on the configuration of the algorithm. By measuring the proportion and ratios of each set of recommendations, we can uncover the configuration of the algorithm, across various context. This configuration gives insight on how each set, and transitively each agent and mechanism that shapes the candidate set, shapes the final recommendations shown to the user. 

\subsection{User Preferences Drive Engagement Decisions} \label{sec:background:user-behavior}
The idea of user agency is central to the discourse on the effects of social media platforms, specifically the content curation algorithms. Where as many problematic recommendations are attributed to bad information consumption patterns of users—there needs to be a deeper investigation of 1) the role user agency plays in the curation of content online, and the 2) multiple layers to user agency that contribute to decisions taken by the users. Specifically in the light of addictive and dysfunctional information consumption patterns. One seminal framework that dissects the user decision making systems proposes a \textit{dual-process} theory. The psychological theory posits that there are two distinct systems in the brain that guide our thinking and decision-making process, System 1 and System 2. The rational ??? system in the processes, System 2 is slow, deliberate and requires conscious effort. It is responsible for active analytical thinking allowing users to evaluate the expected outcomes of their decisions rationally.  System 1, on the other hand, is fast, automatic, and often subconscious. While this guides users through routine tasks and habitual behaviors with minimal cognitive efforts—the system also nudges individuals towards their impulses. Historically, many behavioral economics theories that assume individuals as rational entities—i.e., solely driven by System 2—fail to simulate real user behavior. Deviations from rational models within behavior economics theories are often explainable using the dual-process theory. In our context, as many of the recommendations system are built on behavioral economics theories, they fail to distinguish between the two systems. Simply put, recommendations systems when learning from a user's revealed preferences are unable to distinguish between impulsive preferences and utilitarian preferences. Exploring the outcomes of decisions driven by impulsive preferences reveal the dangers of optimizing for a user's impulse. 

\para{Impulsive information consumption behaviors}
Rise in the spread of misinformation, affective polarization, and confirmation bias are few of many core struggles of the 21st century our society is facing. The underlying mechanisms of these issues can be traced back to our cognitive biases that often dictate our impulses and content consumption. Although these fundamental mechamisms have been present throughout history, their combination with content curation algorithms have constucted dysfunctional feedback loops that reward both the individual and curation algorithms for impulsive content consumption. We argue that current systems, as outlined in our framework, seeking to learn a user's preference are not equipped with the ability to distinguish a user's utilitarian preference from their impulsive preference. Moreover, they might specifically be optimzed to learn a user's impulsive preferences, inadvertently. Since System 1 decisions, i.e. impulsive content consumption, are already faster and subconscious, clearly presenting content that aligns with a user's impulsive preferences, e.g. as the side-bar, with minimal friction in selecting the videos, e.g. automatically playing the next recommended video, we argue content curation algorithm are rewarded by longer engagement by the user and the user experiences minimal cognitive efforts. In other words, we argue YouTube's recommendation algorithm can identify meaningful impulsive preferences of users and reinforce these preferences by serving content that aligns with their preferences.



==> sections/old_sections/introduction.tex <==
\section{Introduction}
Social media platforms have transformed how we consume information. Within these platforms, curated homepages and recommendations have become the primary drivers of content consumption \cite{citation}, making these algorithm drivers for a platform's profitability. Simultaneously, they also play a key role in influencing user behavior and ideologies through shaping their information consumption patterns. In recent years, YouTube's recommendation system has stood out as one of the most critical agents in our socio-political landscape. This is in part due to its vast user base and its engagement with news content \cite{noauthor_social_2024} but also due to its alleged role in disseminating controversial ideologies. There is a rich literature investigating curation and consumption patterns on YouTube for problematic outcomes \cite{brown_echo_2022, chen_subscriptions_2023, haroon_youtube_2022, hosseinmardi_causally_2024, hosseinmardi_examining_2021, liu_algorithmic_2023, munger2022right, noauthor_notitle_nodate, noauthor_notitle_nodate-1, ribeiro_amplification_2023, ribeiro_amplification_2023-1, ribeiro_auditing_2020}, however there is still a gap in understanding what are the fundamental mechanisms through which YouTube makes recommendations, and how these mechanisms might yield problematic patterns. In this work, we uncover how YouTube makes its recommendations by performing a large scale audit of the platform. Then we show, using experimental and observational study design, how recommendations might reinforce problematic user preferences.

\para{Recommendation systems are complex.}
YouTube, similar to other content curation platforms, obtains a large portion of its revenue from advertisement which scale with high user retention \cite{citation}. With the goal to achieve high user retention, YouTube's recommendation algorithms are designed to keep user on the platform, optimizing for engagement. Fundamentally, recommendation algorithms are built with a straightforward task of suggesting content that a user is likely to engage with. These systems leverage behavioral economics theories, which propose that user engagement is met by content that provide utility matching the user's preferences. Although the objectives of a recommendation system are simple, the mechanics used to infer the \textit{utility} of content and the \textit{preferences} of a user render a complex system. Consequently, this system yields recommendations that, while engaging to the user, are shaped by the platform's perception of the user's preferences, and an inferrential understanding of the content's utility developed by the understanding collective user behavior. Therefore, the ultimate curated list of recommended videos is shaped by multiple factors that interact with each other, making any claims for establishing responsibility for problematic recommendations challenging.

\para{Recommendation algorithm construct problematic information exposure patterns.}
Early investigations into recommendation algorithms, specifically YouTube's, discovered emergence of many problematic patterns \cite{ribeiro_auditing_2020}. Initially, these studies often attributed such outcomes to the algorithm itself. However, more recently, investigations have highlighted the significant role user agency play in reinforcing problematic engagement patterns, specifically the user's consumption behaviors—a factor previously under-explored. These conclusions can be explained by considering two key factors. First, the dynamic nature of recommendation algorithms makes them challenging to study consistently over time. Second, and perhaps more significantly, comprehensive takeaways that establish responsibility for problematic outcomes require overcoming the challenge of distinguishing between user agency, algorithmic amplification, and \textit{audience effect}. To this end, we first require an understanding on how recommendations are constructed. This includes questions such as how personalized are recommendations for videos to begin with? and how much of the recommendations dependent on the current video being watched? 

\para{Users have problematic consumption behaviors.}
More complex than recommendation algorithms, are the processes through which individuals make decisions. While systems might expose users to undesirable content or create problematic feedback loops, individuals equally might disproportionately engage with problematic content. Recent studies, using observational studies, have uncovered problematic consumption behaviors driven by users \cite{chen_subscriptions_2023, hosseinmardi_causally_2024}. As recommendations systems seek to estimate and learn user behavior to predict engaging content, these systems learn problematic consumption behaviors that users engage with equally as likely. Therefore, it is important to note the presence of a third additional agency when recommendations are constructed, while the users communicate its preferences through prior interactions, the recommendations system serves recommendations that it predicts to be engaging to the user, the collective users on the platform allow the recommendation system to learn the relationship with user preferences and engaging content. Therefore, preferences that are not present in the collective user behavior will not be reinforced by the algorithm. 

\para{Our Contributions}
While existing studies often demonstrate the presence of problematic patterns, the explanations behind such patterns are left unexplored. In our work, we take a more foundational approach by uncovering how recommendations are constructed and then pursue experiments that showcase how YouTube can reinforce user preferences, including their consumption behavior. First, we illustrate through a framework how recommendations are shaped by three key agents, user preferences, algorithm configurations, and collective user behavior. We then leverage this framework to uncover how YouTube responds to emotional and ideological preferences. Takeaways from these two investigations inform our discussion on the limitations of the preference-utility recommendation framework, responsibility YouTube has to its users, and the influence of collective user behavior on an individual's exposure to content.

\para{RQ1: How personalized are YouTube recommendations?}
Recommendations curated by an algorithm are shaped by many internal and external factors. This includes the user themselves, the configuration of the algorithm, and the collective behavior of the user-base. We investigate how user preferences shape YouTube personalization, more precisely, what proportion of recommendations are driven by personalization. Using a large scale sock-puppet experiment, we assign preferences to sock-puppets which communicate their preferences to YouTube via manipulating their watch history. Subsequently, the sock puppets records one million instances of recommendation as a response. Finally, we represent the recommendations in a latent space. This allows comparison between recommendations shown to different sock puppets for the same videos. We compare recommendations served to sock puppets with assigned preference with recommendations served to sock puppets with no preference to establish level of personalization. This allows explorations into what agencies are involved in serving recommendations—user agency, collective user agency, and algorithmic agency—and how these factors shape the perception of user preferences and content utilities by the platform.

\para{RQ2: Does YouTube reinforce user preferences?}
Recommendation algorithms, when optimized for engagement, seek to infer and reinforce user preferences. While this presents opportunities for the recommendation system to present and curate relevant content for the user, these preferences are a latent features within the system that are not tied with any social or psychological understanding of the preference. We demonstrate, that YouTube recommendation system are unable to distinguish between revealed preferences driven by utility or impulse and therefore reinforce any preference that the user finds engaging. This distinction is important since impulsive consumption of content is more likely to lead to problematic consumption behaviors, addiction, and regret. In our analysis, we design sock puppets with emotional preferences to determine how YouTube responds. More crucially, we uncover how different sources of influence—as identified in RQ1—influence the reinforcing recommendations. Finally, to capture how YouTube responds to more nuanced ideological preferences, we perform an observational study to determine whether users ideological preferences are reinforced from their personalized and contextual recommendations.

Our findings demonstrate how the theoretical framework of recommendations present within YouTube recommendation can construct problematic information exposure patterns. We identify the agents involved in the recommendation system and discuss how their agencies shape responses of the system. Finally, we conclude with observations on how tuning the algorithmic metrics might provide avenues to mitigate problematic recommendations.

==> sections/tables/rq1-method.tex <==

\begin{table}[h!]
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{0.2\textwidth} p{0.5\textwidth} p{0.2\textwidth}}
\toprule
\textbf{Surface} & \textbf{State} & \textbf{Method} \\ \midrule
\multirow{32}{*}{Up-Next} & \multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Personalized: \\ Up-next recommendations observed\\ by the sock-puppet for each of the\\ 100 videos watched.\end{tabular}} & Max \\ \cmidrule(l){3-3} 
 &  & Exposure \\ \cmidrule(l){3-3} 
 &  & Increasing \\ \cmidrule(l){3-3} 
 &  & Rank \\ \cmidrule(l){2-3} 
 & \multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Contextual: \\ Contextual recommendations for the\\ 100 videos watched by the sock-puppet.\end{tabular}} & Max \\ \cmidrule(l){3-3} 
 &  & Exposure \\ \cmidrule(l){3-3} 
 &  & Increasing \\ \cmidrule(l){3-3} 
 &  & Rank \\ \cmidrule(l){2-3} 
 & \multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Blank: \\ Up-next recommendations observed\\ by the sock-puppet without\\ logging in.\end{tabular}} & Max \\ \cmidrule(l){3-3} 
 &  & Exposure \\ \cmidrule(l){3-3} 
 &  & Increasing \\ \cmidrule(l){3-3} 
 &  & Rank \\ \midrule
\multirow{10}{*}{Home} & \multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Personalized: \\ Home page recommendations observed\\ by the sock-puppet after every tenth\\ video watched.\end{tabular}} & Max \\ \cmidrule(l){3-3} 
 &  & Exposure \\ \cmidrule(l){3-3} 
 &  & Increasing \\ \cmidrule(l){3-3} 
 &  & Rank \\ \midrule
\multirow{9}{*}{\begin{tabular}[c]{@{}l@{}}Up-Next\\ Checkpoint\end{tabular}} & \multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Personalized: \\ Up-next recommendations for the starting\\  videos observed by the sock-puppet\\ after every tenth video watched.\end{tabular}} & Max \\ \cmidrule(l){3-3} 
 &  & Exposure \\ \cmidrule(l){3-3} 
 &  & Increasing \\ \cmidrule(l){3-3} 
 &  & Rank \\ \bottomrule
\end{tabular}%
}
\caption{Summary of Recommendations for the Sock-Puppet}
\label{tab:my-table}
\end{table}
